Sampling of the Wiener Process for Remote Estimation over a Channel with Random Delay

In this paper, we consider a problem of sampling a Wiener process, with samples forwarded to a remote estimator over a channel that is modeled as a queue. The estimator reconstructs an estimate of the real-time signal value from causally received samples. We study the optimal online sampling strategy that minimizes the mean square estimation error subject to a sampling rate constraint. We prove that the optimal sampling strategy is a threshold policy, and find the optimal threshold. This threshold is determined by how much the Wiener process varies during the random service time and the maximum allowed sampling rate. Further, if the sampling times are independent of the observed Wiener process, the above sampling problem for minimizing the estimation error is equivalent to a sampling problem for minimizing the age of information. This reveals an interesting connection between the age of information and remote estimation error. Our comparisons show that the estimation error achieved by the optimal sampling policy can be much smaller than those of age-optimal sampling, zero-wait sampling, and periodic sampling.

==> sec_intro__2_.tex <==
% !TEX root = ./sampling_BM.tex
\section{Introduction}

%In remote monitoring and netowcontrol networks, 
%signal sources and estimators are  located in 
%
%
%%\include{sec_related_work}
%
%
%The following are the contributions of this paper:
%\begin{itemize}
%
%\item We formulate an optimal real-time sampling problem for minimizing the causal MSE of the Wiener process, subject to an maximum average sampling rate constraint. %This problem is a constrained continuous-time Markov decision process with a continuous state space, which is usually not easy to solve. 
%The MSE-optimal sampling policy is obtained to resolve this problem. In this MSE-optimal sampling policy, each new sample is generated after all previous samples are delivered. In addition, the generation time of a new sample is determined by both the signal variations since the previous sample and the random transmission delay of the previous sample.  
% 
%\item If the sampling policy is independent of the Wiener process, the MSE minimization problem becomes an age-of-optimization problem 
%
%
%\end{itemize}
%Due to space limitations, all proofs are relegated to our technical report \cite{Sun_reportISIT17}. 
%\subsection{System Model}
%Define the \emph{$\sigma$-fields} $\mathcal{F}_X (t) = \sigma(X(s): s\in[0, t])$ of a continuous-time Markov chain $\{X(t),t\in[0,\infty)\}$. Then, $\{\mathcal{F}_X(t),t\geq0\}$ is the \emph{filtration} (i.e., a growing family of $\sigma$-fields) of $\{X(t),t\in[0,\infty)\}$. A random variable $\tau$ is said to be a \emph{stopping time} of $\{X(t),t\in[0,\infty)\}$, if $\{\tau \leq t\}\in \mathcal{F}_X(t)$ {for all}~$t\geq0$. Define $\mathbb{P}^x(A) = \mathbb{P}(A | X(0) = x)$ and $\mathbb{E}^x Z = \mathbb{E}(Z | X(0) = x)$, respectively, as the conditional probability of event $A$ and the conditional expectation of random variable $Z$ for given initial state $X(0) =x$ of the Markov chain $\{X(t),t\in[0,\infty)\}$. 

%{\red Applications}

In many networked control and monitoring systems (e.g., airplane/vehicular control, smart grid, stock trading, robotics, etc.), real-time updates of the system status state are critical for making decisions, and should be reported to the supervisor or control center in a timely fashion. 
Recently, the \emph{age-of-information}, or simply the \emph{age}, has been proposed as a metric for characterizing  the timeliness of information updates. Suppose that the $i$-th update is generated at time $S_i$ and delivered at time $D_i$. At time $t$, the freshest update delivered to the destination 
was generated at time $\max\{S_i: D_i\leq t\}$. Then, the age at time $t$ is defined as \cite{Song1990,KaulYatesGruteser-Infocom2012}
\begin{align}\label{eq_age_definition}
\age(t)=t- \max\{S_i: D_i\leq t\}. 
\end{align} 
Hence, the age is the \emph{time difference} between the generation time of the freshest received update and the current time $t$.

%between the moment that the freshest delivered update was generated. 

The age-of-information, as well as the general non-linear age penalty models in   \cite{SunInfocom2016,report_AgeOfInfo2016,Bedewy2016,Bedewy2017}, are appropriate for  measuring the timeliness  of \emph{message} updates (e.g., news, fire alarm, email notifications, social updates, etc). However, the status state of  many systems is in the form of a continuous-time signal (e.g., the location/speed/acceleration of a vehicle, the voltage and frequency in an electric power grid, stock price and chart, etc.). The age may not be a perfect metric for evaluating {the timeliness of \emph{signal} updates}. For example, as illustrated in Fig. \ref{fig_signal_eg}, 
a signal may change slow during a time interval and become more dynamic in a later time interval. Hence, the time difference in the age-of-information \eqref{eq_age_definition} is insufficient for precisely characterizing the variability of a signal over time. 

\begin{figure}%[!t]
\centering
%{\subfigure[][The zero-wait policy.]{\resizebox{0.45\textwidth}{!}{\includegraphics{./matlab_SY/example1}}}}
  %  \hspace{0.1\textwidth}
\includegraphics[width=0.45\textwidth]{signal}   
\caption{%Time difference vs signal difference.
Signal variations during time intervals of length $T$.}\vspace{-0.0cm}
\label{fig_signal_eg}
\end{figure}    
 
%which should be reported to a remote controller or monitor
%
%are critical and must be 
%
%
%In  real-time measurements of the system state are reported to the control state in real-time. 
%
%Real-time state measurements are critical for many networked control and monitoring systems, 
%are critical for real-time monitoring and control systems (e.g., )
%
%
%
% measurements are collected and forwarded 
%
%e.g., vichler position tracking, stock-price  , and  real-time signal  are sent thr


In this paper, we investigate timely updates of signal measurements (i.e., signal samples), where the signal is modeled as a Wiener process.
{\blue 
Consider a system with two terminals (see Fig.~\ref{fig_model}): An observer measuring a Wiener process $W_t$ and an estimator, whose goal is to provide the best-guess $\hat W_t$ for the \emph{real-time} value of $W_t$ at every time $t\geq 0$. These two terminals are connected by a channel 
that transmits time-stamped samples of the form $(S_i, W_{S_i})$, where the sampling times $S_i$ satisfy $0\leq S_1 \leq S_2\leq\ldots$ The channel is modeled as a work-conserving FIFO queue with 
%any given non-preemptive service order discipline (e.g., FCFS or LCFS) and 
random \emph{i.i.d.}  delay $Y_i$, where $Y_i\geq 0$ is the channel delay (i.e., random transmission time) of sample $i$.\footnote{By ``work-conserving'', we meant that the channel is kept busy whenever there exist some generated samples that have not been delivered to the estimator.
%This channel model is similar to that considered in \cite{Anantharam1996}. 
} The observer can choose the sampling times $S_i$ causally subject to an average sampling rate constraint
\begin{align} %\label{eq_rate_constraint}
\liminf_{n\to\infty} {1\over n} \mathbb{E}[S_n] \ge {1\over f_{\max}}, \nonumber
\end{align}
where $f_{\max}$ is the maximum allowed sampling rate.} 

Unless it arrives at an empty system, sample $i$ needs to wait  in the queue until its transmission starts. Let $G_i$ be the transmission starting time of sample $i$ such that $S_i \leq G_i$. 
%For any non-preemptive queueing discipline, 
The delivery time of sample $i$ is $D_i = G_i + Y_i$. The initial value $W_0= 0$ is known by the estimator for free, represented by $S_0 =D_0 = 0$. At time $t$, the estimator forms $\hat W_t$ using causally received samples with $D_i \le t$. 
%By minimum mean square error (MSE) estimation,  %\cite{Schervish1995}
%\begin{align}\label{eq_esti}
%\hat{W}_{t}  = & \mathbb{E}[{W}_t | W_{S_j}, D_j \leq t ] \nonumber\\
%                = & W_{S_i}, ~\text{if}~t\in[D_i,D_{i+1}),~i=0,1,2,\ldots, 
%\end{align}
We measure the quality of remote estimation via the mean-square error (MSE) between $W_t$ and $\hat W_t$:
\begin{align}%\label{eq_MSE}
\mathsf{mse} = \limsup_{T\to \infty} {1\over T} \EE \left[\int_0^T (W_t - \hat W_t)^2 dt\right]. \nonumber
\end{align}


%We found that by solving the joint sampling and estimation optimization problem, one can achieve better performance than .

%this enables us to achieve a smaller MSE than age-optimal updates.  
%The optimal sampling problem for minimizing the MSE subject to the  sampling rate constraint is formulated as 



% by solving the following optimal sampling problem.


\begin{figure}%[!t]
\centering
%{\subfigure[][The zero-wait policy.]{\resizebox{0.45\textwidth}{!}{\includegraphics{./matlab_SY/example1}}}}
  %  \hspace{0.1\textwidth}
\includegraphics[width=0.4\textwidth]{example_2}   
\caption{System model.}\vspace{-0.0cm}
\label{fig_model}
\end{figure}    

%\subsection{Contributions} 


%In order to appreciate the difficulty of this joint optimization problem, it is important to comprehend
We study the joint optimization of causal sampling and estimation strategies that achieve the fundamental tradeoff between $f_{\max}$ and $\mathsf{mse}$. 
%We found that by solving this problem, one can achieve a smaller MSE than minimizing the age-of-information. 
One key challenge in this study, and some related work, e.g.,  \cite{Rabi2012,nayyar2013}, is how to optimally convey information to the estimator through samples: A sample $(S_i, W_{S_i})$ naturally reveals the value of the Wiener process $W_t$ at time $t =S_i$. Interestingly, because the sampling time $S_i$ is chosen based on the history observations of $W_t$, a decision on when to generate a sample reveals additional information about $W_t$. For example, if a sample is taken when $W_t>0$, then not receiving a sample for a long time suggests that $W_t$ is likely to be negative. The estimator can use this additional information to reduce the MSE. Accordingly, the sampler  needs to carefully choose the sampling times $S_i$ to make the best usage of the channel and help to reduce the  MSE.


%\footnote{In our case, the $\mathsf{mse}$ is reduced by using this additional information, which will be discussed in Section \ref{sec_signal_independent}. }
 %For example, if no sample has been received for a long time, the estimator can use this knowledge to infer the possible value of $W_t$ reduce its estimation error of $W_t$. 
This, in spirit, is similar to the information theoretic studies in \cite{Gallager1976,Anantharam1996}, where the timing of message arrival times at a queue is used to convey additional information to the receiver. Hence, the Shannon capacity of a queueing system is higher than its service rate $\mu$. 
One difference is that the encoding schemes in \cite{Gallager1976,Anantharam1996} introduce some encoding delay, but we care about \emph{real-time} reconstruction of $W_t$ in this study.  

%Notice that the arrival times of many messages are jointly chosen in \cite{Gallager1976,Anantharam1996}  to achieve the Shannon capacity, which causes a long encoding delay. However, the sampling times $S_i$ in this paper are determined one at a time .   


%, where the timing of wh
%
%the timing of  is used to .
%
%In this paper, we study the joint optimization of the sampling and estimation strategies that achieve the optimal tradeoff between $f_{\max}$ and MSE. In order to appreciate the difficulty of this problem, it is important to understand 
%
%
%information is conveyed to the estimator not only in the contents of the samples, but also in their timing. Because the sampling times $S_i$ are chosen based on the observation of the Wiener process $W_t$, a decision on when to generate a new sample conveys additional information about the Wiener process to the estimator.


%Somewhat to our surprise, we were able to exactly solve \eqref{eq_DPExpected}

\subsection{Contributions}
The  contributions of this paper are summarized as follows:
\ifreport
\begin{itemize}
\else
\begin{itemize}[leftmargin=*]
\fi
\item We formulate the jointly optimal sampling and remote estimation problem as a constrained continuous-time Markov decision problem with a continuous state space, and solve it exactly. 
%It is proven that 
We prove that a threshold-based sampler and a minimum mean-square error (MMSE) estimator are jointly optimal, and the optimal threshold is found.
%the jointly optimal sampling and estimation strategy uses a minimum mean-square error (MMSE) estimation policy and a threshold-based sampling policy, where the optimal threshold is found exactly. 
Let $Y$ be a random variable with the same distribution as $Y_i$. The optimal threshold is determined by $f_{\max}$ and $W_Y$, i.e., the amount of signal variation during the random channel delay. Notice that {$W_Y$ is a random variable that tightly couples the source process $W_t$ and the channel delay $Y$}, which, on a high level, is different from the classic information theory where source coding and channel coding can usually be treated separately.

\item Our threshold-based sampling policy has an important difference from the previous threshold-based sampling policies studied in, e.g., \cite{Astrom2002,Hajek2002,Hajek2008,Lipsa2009, Nuno2011,nayyar2013,Molin2012, ChakravortyTAC2017,imer2010,wu2013,Rabi2012,Basar2014,GaoACC2015, GaoCDC2015, Gao2016,GaoACC2016,GaoAsilomar2016,GaoCDC2016,CHAKRAVORTY2016,ChakravortyISIT2017}: {\blue In our model, each sample waiting in the queue for its transmission opportunity unnecessarily becomes stale. We have proven that it is suboptimal to take a new sample when the channel is busy (using the strong Markov property of the Wiener process). Consequently, the threshold should be \emph{disabled} when the channel is busy and \emph{reactivated} once the channel becomes idle.}

%{\blue In our model, the samples may need to wait  in the queue for their transmission opportunity, and unnecessarily become stale while waiting. We prove that it is suboptimal to take a new sample when the channel is busy transmitting previous samples.  Consequently, the threshold is disabled whenever there is a packet in service.}



%


%As we have mentioned above, the threshold policy in this paper is  different from those of \cite{nayyar2013, wu2013,GaoCDC2015, GaoACC2016,Astrom2002,Basar2014,Chakravorty2015} in the following sense: To avoid the negative effect of queueing, the threshold-based control is disabled until all previous samples are delivered and  is reactivated after that. 


%One of our interesting findings is that the queue should be kept empty at all time such that a new sample is taken only after all previous samples are delivered.


\item An unexpected consequence of our study is that even in the absence of the sampling rate constraint (i.e., $f_{\max}=\infty$), the optimal sampling strategy is \emph{not} zero-wait sampling in which a new sample is generated once the previous sample is delivered; {\blue rather, it is optimal to wait a positive amount of time after the previous sample is delivered, and then take the next sample.}

\item If the sampling times are independent of the observed Wiener process (i.e., the sampling strategy is forced to depend only on the channel but not the source), the joint sampling and estimation optimization problem reduces to an age-of-information optimization problem that has been solved recently \cite{SunInfocom2016,report_AgeOfInfo2016}. The asymptotics of the MSE-optimal and  age-optimal sampling policies at  low/high channel delay or low/high sampling frequencies  are studied. 



\item Our theoretical and numerical comparisons show that the MSE of the optimal sampling policy can be much smaller than those of age-optimal sampling, zero-wait sampling, and classic periodic sampling. In particular, periodic sampling is far from optimal if the sampling rate is low or high; age-optimal  sampling is far from optimal if the sampling rate is low; periodic sampling, age-optimal sampling, and zero-wait sampling policies are all far from optimal if the channel transmission times are highly random.
\end{itemize}

\subsection{Paper Structure}

The rest of this paper is organized as follows. In Section \ref{sec:relate}, we discuss some related work. In Section \ref{sec:model}, we describe
the system model and the formulation of the optimal sampling and remote estimation problem. In Section \ref{sec:solution}, we present the optimal sampling and estimation solution to this problem and compare it with some other sampling policies. In Section \ref{sec_proof}, we describe the proof of this optimal solution. Some simulation results are provided in Section \ref{sec:simulation}.
Finally, in Section \ref{conclusion}, we conclude the 
paper.

\input{sec_related_work_2}



==> sec_related_work.tex <==
% !TEX root = ./sampling_BM.tex
\subsection{Related Work}



On the one hand, the results in this paper are closely related to those in \cite{2015ISITYates,SunInfocom2016,report_AgeOfInfo2016}. Both of these references considered update policies for minimizing the Age-of-information, where update times depend only on the history of the delay process. The discovery of the sub-optimality of a zero-wait policy can be found in these references.

There is a rich literature on remote estimation, e.g., \cite{mehra76, imer2010, nayyar2013, wu2013}. Optimal transmission scheduling of sensor measurements for estimation of a stochastic process was recently studied in \cite{GaoCDC2015, GaoACC2016},  which adopted a finite-horizon formulation with a bound on the total number of transmissions that the sensor can make, over a channel with transmission cost or additive noise. A result in these papers that resonates with ours is the discovery that, under a noisy channel (in contrast to a noiseless one) it may be the case that the sensor does not use all available transmission opportunities. 

In the absence of channel delay and queueing (i.e., $Y_i=0$), the problem   has been addressed
 in \cite{Astrom2002,Basar2014} and the optimality of a threshold policy established. 
As there is no channel delay in the model in \cite{Basar2014},  the problem analyzed therein is a special case of ours with $Y_i$ set to zero for all $i$.  
 
% extend their results to general $Y_i$ and also analyze signal-independent sampling.

%On the other hand, the paper is an extension of the work in \cite{Basar2014}, which considered optimal sampling of a Wiener Process for reconstruction. To our knowledge, this is the first reference that shows that the optimal sampling policy is a threshold policy.  As there is no channel delay in the model in \cite{Basar2014},  the problem analyzed therein is a special case of ours with $Y_i$ set to zero for all $i$. 



==> sec_solution_short.tex <==
% !TEX root = ./sampling_BM.tex


%In this section, we develop a simple optimal sampling policy for solving \eqref{eq_DPExpected}. % by using  martingale, Lagrangian duality, and  optimal stopping theories. % \cite{Shiryaev1978}.

%propose a simple sampling policy and show that it is optimal for 

%Somewhat surprisingly, we find that it is possible to obtain a solution that is optimal for solving \eqref{eq_DPExpected}. % has some nice structural properties that can be exploited to obtain the optimal sample policy. 

% in the sequel.
%In this section, we will solve \eqref{eq_DPExpected} by using 
%\subsection{Problem Simplification} % 
%\begin{lemma}
%Let $S\leq T$ be two stopping times of the Wiener process $W_t$ and $\mathbb{E}[T]<\infty$. Then
%\begin{align}
%\mathbb{E}\left[ W_t^4 \right] = \mathbb{E}\left[ W_s^4 \right] + \mathbb{E}\left[ (W_t- W_s)^4 \right].  
%\end{align}
%\end{lemma}
%If a sample is stored in the queue, it becomes stale while waiting for its transmission opportunity. 
%A better method is to wait until the channel becomes idle, and then generate a new sample. This completely eliminates the waiting time wasted in the queue, and hence the queue is kept empty. 
%
%\begin{lemma}\label{lem_zeroqueue}
%In \eqref{eq_DPExpected}, it is better to take samples only when the channel is idle. 
%\end{lemma}
%\begin{proof}
%See Appendix \ref{app_zeroqueue}. 
%\end{proof}
%By Lemma \ref{lem_zeroqueue}, we only need to consider a sub-class of sampling policies $\Pi_1\subset\Pi$ such that each  sample is generated and submitted to the channel after all previous samples are delivered, i.e., 
%\begin{align}
%\Pi_1 = \{\pi\in\Pi: S_{i} = G_{i} \geq D_{i-1} \text{ for all $i$}\}. \nonumber
%\end{align}%In particular, sample $i$ is delivered before sample $i+1$ is generated and sent out, i.e., $D_{i} \leq S_{i+1} = G_{i+1}$. 
%Hence, the \emph{information} that is available for determining $S_i$ includes the history of signal values $(W_t: t\in[0, S_i])$ and the transmission delays  $(Y,\ldots, Y_{i-1})$ of previous samples. To characterize this statement precisely, let us define the $\sigma$-field $\mathcal{F}_t = \sigma(W_s: s\in[0, t])$. Then, $\{\mathcal{F}_t,t\geq0\}$ is the {filtration} (i.e., a growing family of $\sigma$-fields) of the Wiener process $W_t$.
%%, and $\{\mathcal{F}_C (i), i = 1,2,\ldots\}$ is the \emph{filtration} of the channel transmission process. Then, 
%Given the transmission  durations $(Y,\ldots, Y_{i-1})$ of previous samples, $S_{i} $ is a \emph{stopping time} with respect to the filtration $\{\mathcal{F}_t,t\geq0\}$ of the Wiener process $W_t$, that is
%\begin{align}
%[\{S_{i}\leq t\} | Y,\ldots, Y_{i-1}] \in \mathcal{F}_t.\label{eq_stopping}
%\end{align}  
%Then, the policy space $\Pi_1$ can be expressed as
%\begin{align}\label{eq_policyspace}
%\!\!\!\!\Pi_1 = & \{S_i : [\{S_{i}\leq t\} | Y,\ldots, Y_{i-1}] \in \mathcal{F}_t, \nonumber\\
%&\text{$T_i$ is a regenerative process} \}.\!\!
%\end{align}  
%%This %interpretation 
%% which will be used to simplify \eqref{eq_DPExpected}:
%% for simplifying \eqref{eq_DPExpected}. %  which we obtain  the following result:
%%This interpretation motivated us to 
%
%Using the stopping times and martingale theory of Wiener process, we obtain the following  lemma 
%%
%that is useful for simplifying \eqref{eq_DPExpected}: %that is obtained along this direction 
%%is the following lemma:
%\begin{lemma}\label{lem_stop}
%Let $\tau \geq0$ be a stopping time of the Wiener process $W_t$ with $\mathbb{E}[\tau^2]<\infty$, 
%then
%\begin{align}\label{eq_stop}
%%\mathbb{E}\left[\int_0^T [{x}(0)-W_t]^2dt\right] = \mathbb{E}[T] \sigma^2.
%\mathbb{E}\left[\int_0^\tau W_t^2 dt\right]= \frac{1}{6}\mathbb{E}\left[ W_\tau^4 \right].
%\end{align}
%\end{lemma}
%\begin{proof}
%See Appendix \ref{applem_stop}.
%\end{proof}
%
%%From \eqref{eq_esti}, we can get
%%\begin{align}%\label{eq_integral}
%%\mathbb{E}\!\left\{
%%\!\int_{D_{i}}^{D_{i+1}} \!\![W_t\!-\!\hat W_t]^2dt\right\}\!{=} \mathbb{E}\!\left\{\!\int_{D_{i}}^{D_{i+1}} \! \![W_t\!-\!B(S_{i})]^2dt\right\}\!.\! \nonumber
%%\end{align}
%
%
%Let $Z_i = S_{i+1} - D_{i}\geq0$ represent the \emph{waiting time} between the delivery time $D_{i}$ of sample $i$  and the generation time $S_{i+1}$ of sample $i+1$. Then,
%$S_i =  Z_{0} +\sum_{j=0}^{i-1} (Y_{j} + Z_j)$ and $D_i =  \sum_{j=0}^{i-1} (Z_{j}+Y_{j+1})$. If $(Y,Y_2,\ldots)$ is given, $(S_0,S_1,\ldots)$ is uniquely determined by $(Z_0,Z_1,\ldots)$. Hence, one can also use $\pi = (Z_0,Z_1,\ldots)$ to represent a sampling policy. 
%% For the convenience of later discussions, we will use $\pi = (Z_0,Z_1,\ldots)$ to represent a sampling policy in the sequel. 
%%Let 
%%\begin{align}\label{eq_shift}
%%W_{s+t}-W_{s} = W_{s+t}-W_s, ~s,t\geq0,
%%\end{align}
%%represent the signal variation since time $s$. According to  \cite[Theorem 2.16]{BMbook10}, $W_{s+t}-W_{s}$ is also a  Wiener process, called \emph{time-shifted Wiener process}. 
%
%
%%  we can show that for every $i = 1,2,\ldots$,
%%\begin{align}\label{eq_integral}
%%&\mathbb{E}\left\{\int_{D_{i}}^{D_{i+1}} [W_t-\hat W_t]^2dt\right\} \nonumber\\
%%%=& \mathbb{E}\left\{\int_{D_{i}}^{D_{i+1}} [W_t-B(S_i)]^2dt\right\} \nonumber\\
%%%= & \mathbb{E}\left\{\int_{Y_i}^{Y_i+Z_i+Y_{i+1}} W_t^2dt\right\} \nonumber\\
%%%= & \frac{1}{6}\mathbb{E}\left[ B(Y_i+Z_i+Y_{i+1})^4 \right] - \frac{1}{6}\mathbb{E}\left[ B(Y_i)^4 \right] \nonumber\\
%%= & \frac{1}{6}\mathbb{E}\left[ (W_{S_{i}+Y_i+Z_i}-W_{S_i})^4 \right] + \mathbb{E}\left[Y_i + Z_i \right] \mathbb{E}\left[Y_i \right],  
%%\end{align}
%%which is proven in Appendix \ref{app_integral}.
%%%%In addition, the following result is crucial for simplifying : 
%%%\begin{lemma}\label{lem_ergodic}
%%%For the Wiener process $W_t$, if $\{S_{i+1}-S_i, i = 0,1,\ldots\}$ is ergodic, then $\{B(S_{i+1})-B(S_i), i = 0,1,\ldots\}$ is ergodic.
%%%\end{lemma}
%%%\begin{proof}
%%%%For notational simplicity, denote $C_i = S_{i+1}-S_i$ and $D_i = B(S_{i+1})-B(S_i)$. 
%%%Because of Kolmogorov's extension theorem \cite[Theorem A.3.1]{Durrettbook10}, there exists a probability space $(\Omega, \mathcal{F}, P)$ with $\Omega = \mathbb{R}^{\{0,1,\ldots\}}$ and $\omega= (\omega_0, \omega_1,\ldots)\in \Omega$ such that the sequence $C_i(\omega) = \omega_i$ has the same distribution as that of $\{S_{i+1}-S_i, i=0,1,\ldots\}$. 
%%%Let $\varphi: \Omega \mapsto \Omega$ be the shift operator such that $\varphi(\omega_0, \omega_1,\ldots) = (\omega_1, \omega_2,\ldots)$, and let $C(\omega) = \omega_0$. Hence, $C_i(\omega) = C(\varphi^i \omega)$. Because $\{S_{i+1}-S_i, i = 0,1,\ldots\}$ is ergodic, $\varphi$ is measure preserving, i.e., $P[\varphi^{-1} A] = P[A]$ for all $A\in \mathcal{F}$.
%%%%Then,   measurable mapping $$ such that   where $C$ is a random variable. 
%%%
%%%See Appendix \ref{applem_ergodic}.
%%%\end{proof}
%%%Because the $Y_i$'s are \emph{i.i.d.} and 
%%Because $T_i $ is a regenerative process, the renewal theory \cite{Ross1996} tells us that $\frac{1}{n} 
%%\mathbb{E}[S_n]= \frac{1}{n} 
%%\sum_{i=1}^n \mathbb{E}\left[Y_i+Z_i\right]$ is a convergent seqence and %$(Z_1,Z_2,\ldots)$ is also stationary and ergodic. Hence, 
%%%Because  $(Y,Y_2,\ldots)$ are \emph{i.i.d.} and $(Z_1,Z_2,\ldots)$ are stationary and ergodic, we can obtain
%%\begin{align}
%%&\limsup_{T\rightarrow \infty}\frac{1}{T}\mathbb{E}\left\{\int_0^{T} [W_t-\hat W_t]^2dt\right\} \nonumber
%%\\
%%=& \lim_{n\rightarrow \infty}\frac{\mathbb{E}\left\{\int_0^{D_n} [W_t-\hat W_t]^2dt\right\}}{\mathbb{E}[D_n]} \nonumber\\
%%=& \lim_{n\rightarrow \infty}\frac{\sum_{i=1}^n\!\! \left\{\mathbb{E}\left[(W_{S_{i}+Y_i+Z_i}\!-\!W_{S_i})^4\right]\!+\! 6\mathbb{E}\left[Y_i+Z_i\right]\mathbb{E}\left[Y_i\right]\right\}}{6\sum_{i=1}^n \mathbb{E}\left[Y_i+Z_i\right]}\nonumber\\
%%= & \lim_{n\rightarrow \infty}\frac{\sum_{i=1}^n\mathbb{E}\left[(W_{S_{i}+Y_i+Z_i}-W_{S_i})^4\right]}{ 6\sum_{i=1}^n \mathbb{E}\left[Y_i+Z_i\right]} +  \mathbb{E}\left[Y\right],\nonumber
%%\end{align}
%%where we have used $\mathbb{E}\left[D_n\right]=\mathbb{E}[\sum_{i=0}^{n-1} (Z_{i}+Y_{i+1})] = \mathbb{E}[\sum_{i=0}^{n-1} (Y_{i}+Z_{i})]$ and $\mathbb{E}\left[Y_i\right] = \mathbb{E}\left[Y\right]$.
%%Hence, 
%Using Lemma \ref{lem_stop}, \eqref{eq_DPExpected} can be rewritten as the following Markov decision process:
%\begin{align}\label{eq_Simple}
%&\min_{\pi\in\Pi_1} \lim_{n\rightarrow \infty}\frac{\sum_{i=1}^n\mathbb{E}\left[(W_{S_{i}+Y_i+Z_i}-W_{S_i})^4\right]}{ 6\sum_{i=1}^n \mathbb{E}\left[Y_i\!+\!Z_i\right]} \!+\!  \mathbb{E}\left[Y\right] \\
%&~\text{s.t.}~\lim_{n\rightarrow \infty} \frac{1}{n} 
%\sum_{i=1}^n \mathbb{E}\left[Y_i+Z_i\right]\geq \frac{1}{f_{\max}},\nonumber
%\end{align}
%where ${\mathsf{mmse}}_{\text{opt}}$ is the optimal  value of \eqref{eq_Simple}. 
%
%
%\subsection{Dual Decomposition with Zero Duality Gap}
%In order to solve \eqref{eq_Simple}, let us consider the following Markov decision process with a parameter $c\geq 0$:
%%In order to solve \eqref{eq_Simple}, let us consider the following Markov decision with a parameter $c$:
%\begin{align}\label{eq_SD}
%\!\!\!\!\!\!f(c)\!=\!\min_{\pi\in\Pi_1}&\lim_{n\rightarrow \infty}\frac{1}{n}\sum_{i=1}^n\!\mathbb{E}\!\left[\frac{1}{6}(W_{S_{i}+Y_i+Z_i}\!-\!W_{S_i})^4\!-\! c(Y_i\!+\!Z_i)\!\right]\!\!\!\!\\
%\text{s.t.}~&\lim_{n\rightarrow \infty} \frac{1}{n} 
%\sum_{i=1}^n \mathbb{E}\left[Y_i+Z_i\right]\geq \frac{1}{f_{\max}},\nonumber
%\end{align}
%where $f(c)$ is the optimum  value of \eqref{eq_SD}. 
%\begin{lemma} \label{lem_ratio_to_minus}
%The following assertions are true:
%\begin{itemize}
%\vspace{0.5em}
%\item[(a).] \emph{${\mathsf{mmse}}_{\text{opt}} \gtreqqless c +  \mathbb{E}\left[Y\right]$} if and only if $f(c)\gtreqqless 0$. 
%\vspace{0.5em}
%\item[(b).] If $f(c)=0$, the solutions to \eqref{eq_Simple}
%and \eqref{eq_SD} are identical. 
%\end{itemize}
%\end{lemma}
%\begin{proof}
%See Appendix \ref{app_ratio_to_minus}.
%\end{proof}
%Hence, the solution to \eqref{eq_Simple} can be obtained by solving \eqref{eq_SD} and seeking a parameter $c\geq 0$ such that 
%\begin{align}\label{eq_c}
%f(c)=0.
%\end{align}
%
%Although \eqref{eq_SD} is not a convex optimization problem, it is possible to use the Lagrangian dual approach to solve \eqref{eq_SD} and show that it admits no duality gap. 
%
%%Specifically, define the following Lagrangian function
%%\begin{align}
%%& L(\pi;\lambda) \nonumber\\
%%=& \lim_{n\rightarrow \infty}\frac{1}{n}\sum_{i=1}^n\mathbb{E}\left[\frac{1}{6}(W_{S_{i}+Y_i+Z_i}-W_{S_i})^4\!-\! (c+\lambda)(Y_i\!+\!Z_i)\right] \nonumber\\
%%&+ \frac{\lambda}{f_{\max}}.\nonumber
%%\end{align}
%%Let
%%\begin{align}\label{eq_primal}
%%g(\lambda) = \inf_{\pi\in\Pi_1}  L(\pi;\lambda).
%%\end{align}
%%Then, the Lagrangian dual problem of \eqref{eq_SD} is defined by
%%\begin{align}\label{eq_dual}
%%\max_{\lambda\geq 0}g(\lambda).
%%\end{align}
%%Similar with \cite{Yu2006,Luo2008}, strong duality can be established as
%%\begin{lemma}\label{thm_zero_gap}
%%The optimal values of \eqref{eq_SD} and \eqref{eq_dual} are equal; i.e., their duality gap is zero.
%%\end{lemma}
%%\begin{proof}
%%See Appendix \ref{app_zero_gap}.
%%\end{proof}
%Define the $\sigma$-field $\mathcal{F}^{s}_t = \sigma(W_{s+v}-W_{s}: v\in[0, t])$ and the {filtration} $\{\mathcal{F}^{s}_t,t\geq0\}$ of the {time-shifted Wiener process} $\{W_{s+t}-W_{s},t\in[0,\infty)\}$. In addition, define ${\mathfrak{M}}_s$ as the set of square-integrable stopping times of $\{W_{s+t}-W_{s},t\in[0,\infty)\}$, i.e.,
%\begin{align}
%\mathfrak{M}_{s} = \{\tau \geq 0:  \{\tau\leq t\} \in \mathcal{F}^{s}_t, \mathbb{E}\left[\tau^2\right]<\infty\}.\nonumber
%\end{align}
%Let 
%\begin{align}
%\beta = 3(c + \lambda).\nonumber
%\end{align}
%By using Lemma \ref{lem_ratio_to_minus}, Lemma \ref{thm_zero_gap}, and the sufficient statistics of the Markov decision process \eqref{eq_primal}, we get
%\vspace{-1em}
\section{Proof Sketch of the Main Result}\label{sec_proof}
A proof sketch of Theorem~\ref{thm_1} is provided here, and the detailed proof is relegated to our technical report \cite{Sun_reportISIT17}: 

We first provide a lemma that is crucial for simplifying \eqref{eq_DPExpected}.

\begin{lemma}\label{lem_zeroqueue}
%In the optimal sampling problem \eqref{eq_DPExpected} for minimizing the MMSE of the Wiener process, it is suboptimal to take a new sample before the previous sample is delivered. 
In the optimal sampling problem \eqref{eq_DPExpected} for minimizing
the MMSE of the Wiener process, it is suboptimal to take a new sample before the previous sample is delivered.
%In the optimal sampling problem \eqref{eq_DPExpected} for minimizing the MMSE of the Wiener process, it is better to wait until the channel becomes idle, and then generate each new sample and immediately send it out.
\end{lemma}

%Unless it arrives at an empty system, sample $i$ needs to wait  in the queue until its transmission starts. 

{\blue In recent studies on age-of-information  \cite{SunInfocom2016,report_AgeOfInfo2016}, Lemma \ref{lem_zeroqueue} was intuitive and hence was used without a proof: If a sample is taken when the channel is busy, it needs to wait in the queue until its transmission starts, and becomes stale while waiting. A better method is 
to wait until the channel becomes idle, and then generate a new
sample, as stated in Lemma \ref{lem_zeroqueue}. However, this lemma is not intuitive in the MMSE minimization problem \eqref{eq_DPExpected}: The proof of Lemma \ref{lem_zeroqueue} relies on the strong Markov property of Wiener process, which may not hold for other signal processes. 
}
%\begin{proof}
%See Appendix \ref{app_zeroqueue}. 
%\end{proof}

By Lemma \ref{lem_zeroqueue}, we only need to consider a sub-class of sampling policies $\Pi_1\subset\Pi$ defined by 
%such that each  sample is generated and submitted to the channel after all previous samples are delivered, i.e., 
\begin{align}
\Pi_1 = \{\pi\in\Pi: S_{i+1} = G_{i+1} \geq D_{i} \text{ for all $i$}\}. \nonumber
\end{align}
This completely eliminates the waiting time wasted in the queue, and hence the queue should always be kept empty.
Let $Z_i = S_{i+1} - D_{i}\geq0$ represent the \emph{waiting time} between the delivery time $D_{i}$ of sample $i$  and the generation time $S_{i+1}$ of sample $i+1$. Then,
$S_i =  Z_{0} +\sum_{j=1}^{i-1} (Y_{j} + Z_j)$ and $D_i =  \sum_{j=0}^{i-1} (Z_{j}+Y_{j+1})$ for each $i=1,2,\ldots$ If $(Y_1,Y_2,\ldots)$ is given, $(S_0,S_1,\ldots)$ is uniquely determined by $(Z_0,Z_1,\ldots)$. Hence, one can also use $\pi = (Z_0,Z_1,\ldots)$ to represent a sampling policy. 

Because $T_i $ is a regenerative process, \eqref{eq_DPExpected} can be reformulated as the following Markov decision problem:
\begin{align}\label{eq_Simple}
{\mathsf{mmse}}_{\text{opt}}\triangleq&\min_{\pi\in\Pi_1} \lim_{n\rightarrow \infty}\frac{\sum_{i=0}^{n-1}\mathbb{E}\left[\int_{D_{i}}^{D_{i+1}} (W_t\!-\!W_{S_{i}})^2dt\right]}{\sum_{i=0}^{n-1} \mathbb{E}\left[Y_i+Z_i\right]} \\
&~\text{s.t.}~\lim_{n\rightarrow \infty} \frac{1}{n} 
\sum_{i=0}^{n-1} \mathbb{E}\left[Y_i+Z_i\right]\geq \frac{1}{f_{\max}},\label{eq_Simple_constraint}
\end{align}



Define the $\sigma$-fields $\mathcal{F}^{s}_t = \sigma(W_{s+v}-W_{s}: v\in[0, t])$ and $\mathcal{F}^{s+}_t = \cap_{v>t} \mathcal{F}^{s}_v$, as well as the {filtration} (i.e., a non-decreasing and right-continuous  family of  $\sigma$-fields) $\{\mathcal{F}^{s+}_t,t\geq0\}$ of the {time-shifted Wiener process} $\{W_{s+t}-W_{s},t\in[0,\infty)\}$. Let ${\mathfrak{M}}_s$ denote the set of square-integrable stopping times of $\{W_{s+t}-W_{s},t\in[0,\infty)\}$, i.e.,
\begin{align}
\mathfrak{M}_{s} = \{\tau \geq 0:  \{\tau\leq t\} \in \mathcal{F}^{s+}_t, \mathbb{E}\left[\tau^2\right]<\infty\}.\nonumber
\end{align}
After some manipulations, we formulate the Lagrangian dual problem of \eqref{eq_Simple}, which can be 
decomposed into a sequence of \emph{mutually independent} per-sample control problem \eqref{eq_opt_stopping}:
\begin{align}\label{eq_opt_stopping}
Z_i =&  \min_{\tau  \in \mathfrak{M}_{S_i+Y_i}} \mathbb{E}\left[\frac{1}{2}(W_{S_{i}+Y_i+\tau}-W_{S_i})^4\right.\nonumber\\
&~~~~~~~~~~~~~~~~\left.- {\beta}(Y_i+\tau)\bigg|W_{S_{i}+Y_i}-W_{S_i},Y_i \right],
\end{align}
where $\beta\geq0$ is the dual variable. In the proof of \eqref{eq_opt_stopping}, we have used 
%Next, by using the stopping times and martingale theory of Wiener process, we obtain 
the following lemma: 
%
%that is useful for rewritten \eqref{eq_DPExpected} as a Markov decision process without integral: %that is obtained along this direction 
%is the following lemma:
\begin{lemma}\label{lem_stop}
Let $\tau \geq0$ be a stopping time of the Wiener process $W_t$ with $\mathbb{E}[\tau^2]<\infty$, 
then
\begin{align}\label{eq_stop}
%\mathbb{E}\left[\int_0^T [{x}(0)-W_t]^2dt\right] = \mathbb{E}[T] \sigma^2.
\mathbb{E}\left[\int_0^\tau W_t^2 dt\right]= \frac{1}{6}\mathbb{E}\left[ W_\tau^4 \right].
\end{align}
\end{lemma}

Using the optimal stopping rule developed in \cite{Shiryaev1978}, we get 
\begin{theorem}
An optimal solution to \eqref{eq_opt_stopping} is
\begin{align}\label{eq_opt_stop_solution1}
Z_i = \inf \left\{ t \geq 0:\! \left|W_{S_i+Y_i+t}-W_{S_i}\right| \geq \sqrt{\beta}\right\}.
\end{align}
\end{theorem}
Notice that \eqref{eq_opt_stop_solution1} is equivalent to \eqref{eq_opt_solution}. 
\begin{theorem}\label{thm_zero_gap}
The following assertions are true:
\begin{itemize}
\item[(a).] The duality gap between \eqref{eq_Simple} and its Lagrangian dual problem is zero.
\item[(b).] A common optimal solution to \eqref{eq_DPExpected} and  \eqref{eq_Simple} is given by \eqref{eq_opt_solution} and \eqref{eq_thm1}. 
\end{itemize}
%Hence, the MMSE-optimal  policy in \eqref{eq_opt_solution} and \eqref{eq_thm1} is an optimal solution to \eqref{eq_SD}. 
\end{theorem}
By this, Theorem~\ref{thm_1} is proven.
%the duality gap between \eqref{eq_Simple} and its Lagrangian dual problem is zero, and the optimal $\beta$ is determined by \eqref{eq_thm1}. 


\ignore{



\begin{theorem}\label{thm_solution_form}
An optimal solution to \eqref{eq_Simple}
%, or equivalently \eqref{eq_c}-\eqref{eq_dual}, 
satisfies


%is determined by solving
%\begin{align}\label{eq_equation}
%\mathbb{E}[Y_i+Z_i] \!=\! \max\left(\frac{1}{f_{\max}}, \frac{\mathbb{E}[(W_{S_{i}+Y_i+Z_i}-W_{S_i})^4]}{2\beta}\right).\!
%\end{align}
%The optimal  value of \eqref{eq_Simple} is then given by \emph{
%\begin{align}\label{thm_3_obj}
%\mathsf{mmse}_{\text{opt}}=\frac{\mathbb{E}[(W_{S_{i}+Y_i+Z_i}-W_{S_i})^4]}{6\mathbb{E}[Y_i+Z_i] } + \mathbb{E}[Y].
%\end{align}}
\end{theorem}



Note that 
the expectations in \eqref{eq_equation} and \eqref{thm_3_obj} remain constant for all $i=1,2,\ldots$, as shown in \cite{Sun_reportISIT17}. Finally,  \eqref{eq_opt_stopping} is solved by using the optimal stopping rule developed in  \cite{Shiryaev1978}.
%\begin{proof}
%See Appendix \ref{app_solution_form}. 
%\end{proof}
%By this, 
% and the optimal $\alpha$ is given by \eqref{eq_equation}.

%\subsection{Per-sample Optimal Stopping Rule}


%Let us first pose \eqref{eq_opt_stopping} in the language of  optimal stopping.
%A continuous-time two-dimensional Markov chain $X_t$ on a probability space $(\mathbb{R}^2,\mathcal{F},\mathbb{P})$ is defined as follows:  Given the initial state $ X_0=x = (s,b)$, the state $X_t$ at time $t$ is  
%\begin{align}\label{eq_Markov}
%X_t= (s + t, b + W_t), 
%\end{align}
%where $\{W_t,t\geq 0\}$ is a standard Wiener process. 
%%Define $\mathbb{P}^x(A) = \mathbb{P}(A | X_0 = x)$ and $\mathbb{E}^x Z = \mathbb{E}(Z | X_0 = x)$, respectively, 
%%as the conditional probability of event $A$ and the conditional expectation of random variable $Z$ 
%%for given  initial state $X_0 =x$. 
%Define the $\sigma$-field $\mathcal{F}^{X}_t  = \sigma(X_{v}: v\in[0, t])$ and the {filtration} $\{\mathcal{F}^{X}_t ,t\geq0\}$ of the Markov chain $X_t$.
%A random variable $\tau: \mathbb{R}^2\rightarrow [0,\infty)$ is said to be a \emph{stopping time} of $X_t$ if $\{\tau \leq t\}\in \mathcal{F}^{X}_t $ {for all}~$t\geq0$. Let ${\mathfrak{M}}$ be the set of  square-integrable stopping times of $X_t$, i.e.,
%\begin{align}
%\mathfrak{M} = \{\tau \geq 0:  \{\tau\leq t\} \in \mathcal{F}^{X}_t , \mathbb{E}\left[\tau^2\right]<\infty\}.\nonumber
%\end{align}

%Let $\{\mathcal{F}(t),t\geq0\}$ be a \emph{filtration} of the process $\{X(t),t\geq 0\}$, that is, a family of $\sigma$-fields 
%$\mathcal{F}(t) = \sigma(X(s):0\leq s \leq t)$ such that $\mathcal{F}(s) \subset \mathcal{F}(t)  \subset \mathcal{F}$ for all $0\leq s< t$. 
%A random variable $\tau: \mathbb{R}^2\rightarrow [0,\infty]$ is said to be a \emph{stopping time} with respect to the filtration $\{\mathcal{F}(t),t\geq0\}$ if $\{\tau \leq t\}\in \mathcal{F}(t)$ {for all}~$t\geq0$.
%Let $\overline{\mathfrak{M}}$ be the set of all stopping times and $\mathfrak{M}$ be the set of all finite stopping times, i.e.,\begin{align}
%\mathfrak{M} = \{\tau\in \overline{\mathfrak{M}}: \mathbb{P}^x(\tau<\infty) = 1,~\forall~x\in \mathbb{R}^2\}.
%\end{align}
%Our goal is to solve the following optimal stopping problem:
%\begin{align}\label{eq_stop_prob}
%\sup_{\tau\in \mathfrak{M}}  \mathbb{E}^x g(X_\tau),
%\end{align}
%where the function $g: \mathbb{R}^2\rightarrow \mathbb{R}$ is defined as 
%\begin{align}\label{eq_fun}
%g(s,b) = - \frac{1}{2}b^4+\beta s 
%\end{align}
%with parameter $\beta \geq 0$, and $x$ is the initial state of the Markov chain $X(t)$. Note that \eqref{eq_stop_prob} reduces to \eqref{eq_opt_stopping}
%if the initial state is $ x=(Y_i,W_{S_{i}+Y_i}-W_{S_i})$,  and  $W_t$ is replaced by $W_{S_{i}+Y_i+t}-W_{S_i}$. 
%By using the optimal stopping theory of Markov chain \cite{Shiryaev1978,Peskir2006}, we establish the following result:
%\begin{theorem}\label{thm_optimal_stopping}
%For any initial state $(s,b)\in \mathbb{R}^2$, an optimal stopping time for solving \eqref{eq_stop_prob} is
%\begin{align}\label{eq_opt_stop_solution}
%\tau^* = \inf \left\{ t \geq 0:\! \left|b+W_t\right| \!\geq\! \sqrt{\beta}\right\}.
%\end{align}
%\end{theorem} 
%\begin{proof}
%See our technical report \cite{Sun_reportISIT17}.
%\end{proof}
%We will prove Theorem \ref{thm_optimal_stopping} by using the optimal stopping theory of Markov chain \cite{Shiryaev1978,Peskir2006}. To that end, 

%In order to prove Theorem \ref{thm_optimal_stopping}, let us define the function
%$u(x) = \mathbb{E}^x g(X_{\tau^*})$ and establish some properties of $u(x)$.
%
%\begin{lemma} \label{lem1_stop}
% $u(x)\geq g(x)$ for all $x\in \mathbb{R}^2$, and 
%\begin{align}
%u(s,b) = \left\{\begin{array}{l l} 
%\beta s- \frac{1}{2}b^4 , &\text{if}~ b^2 \geq \beta;
%\vspace{0.5em}\\
%\beta s+ \frac{1}{2} \beta ^2- \beta b^2 , &\text{if}~ b^2 < \beta.
%\end{array}\right.
%\end{align}
%\end{lemma} 
%\begin{proof}
%See Appendix \ref{app_optimal_stopping}. 
%\end{proof}
%
%A function $f(x)$ is said to be \emph{excessive} for the process $X_t$ if \cite{Shiryaev1978}
%\begin{align}
%\mathbb{E}^x f(X_t)\leq f(x),~\text{for all}~ t\geq 0, ~x\in \mathbb{R}^2.
%\end{align} 
%By using It\^{o} and Tanaka's formula in stochastic calculus, we can obtain
%\begin{lemma}\label{lem2_stop}
%The function $u(x)$ is excessive for the process $X_t$.
%\end{lemma} 

%
%\begin{proof}
%See Appendix \ref{app_optimal_stopping1}. 
%\end{proof}
%
%Now, we are ready to prove Theorem \ref{thm_optimal_stopping}. 
%\begin{proof}[Proof of Theorem \ref{thm_optimal_stopping}]
%In Lemma \ref{lem1_stop} and Lemma \ref{lem2_stop}, we have shown that $u(x)=\mathbb{E}^x g(X_{\tau^*})$ is an excessive function and $u(x)\geq g(x)$. In addition, it is known that $\mathbb{P}^x(\tau^*<\infty) = 1$ for all $x\in \mathbb{R}^2$ \cite[Theorem 8.5.3]{Durrettbook10}. These conditions, together with the Corollary to Theorem 1 in \cite[Section 3.3.1]{Shiryaev1978}, imply that $\tau^*$ is an optimal stopping time of \eqref{eq_stop_prob}. This completes the proof.
%\end{proof}


%An immediate consequence of Theorem \ref{thm_optimal_stopping} is
\begin{theorem}\label{coro_stop}
An optimal solution to \eqref{eq_opt_stopping} is
\begin{align}\label{eq_opt_stop_solution1}
Z_i = \inf \left\{ t \geq 0:\! \left|W_{S_i+Y_i+t}-W_{S_i}\right| \!\geq\! \sqrt{\beta}\right\},
\end{align}
and the expectations in \eqref{eq_equation} and \eqref{thm_3_obj} are then given by
\begin{align}
&\mathbb{E}[Y_i+Z_i] = \mathbb{E}[\max(\beta,W_Y^2)],\label{eq_expression0}\\
&\mathbb{E}[(W_{S_{i}+Y_i+Z_i}-W_{S_i})^4] = \mathbb{E}[\max(\beta^2,W_Y^4)].\label{eq_expression}
\end{align}
\end{theorem}
Combining Theorem \ref{thm_solution_form} and Theorem \ref{coro_stop}, Theorem~\ref{thm_1} follows.}
%Finally, \eqref{eq_expression0} and \eqref{eq_expression} are proven in Appendix \ref{app_expression}. 
%This completes the proof of Theorem \ref{thm_1}.


